Random Forest with Learned Representations for Semantic Segmentation

In this work, we present a random forest framework that learns the weights, shapes, and sparsities of feature representations for real-time semantic segmentation. Typical filters (kernels) have predetermined shapes and sparsities and learn only weights. A few feature extraction methods fix weights and learn only shapes and sparsities. These predetermined constraints restrict learning and extracting optimal features. To overcome this limitation, we propose an unconstrained representation that is able to extract optimal features by learning weights, shapes, and sparsities. We, then, present the random forest framework that learns the flexible filters using an iterative optimization algorithm and segments input images using the learned representations. We demonstrate the effectiveness of the proposed method using a hand segmentation dataset for hand-object interaction and using two semantic segmentation datasets. The results show that the proposed method achieves real-time semantic segmentation using limited computational and memory resources.

==> fig_RF_PSO.tex <==
\begin{figure}[!t] \begin{center}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[scale=0.25]{fig/empty.jpg}}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[scale=0.25]{fig/empty.jpg}}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[scale=0.25]{fig/empty.jpg}}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[scale=0.25]{fig/empty.jpg}}
\end{minipage}
   \caption{An example of particle swarm optimization.}
\label{fig:PSO}
\end{center}\end{figure}


